Automating Vascular Shunt Insertion with the dVRK Surgical Robot

Vascular shunt insertion is a fundamental surgical procedure used to temporarily restore blood flow to tissues. It is often performed in the field after major trauma. We formulate a problem of automated vascular shunt insertion and propose a pipeline to perform Automated Vascular Shunt Insertion (AVSI) using a da Vinci Research Kit. The pipeline uses a learned visual model to estimate the locus of the vessel rim, plans a grasp on the rim, and moves to grasp at that point. The first robot gripper then pulls the rim to stretch open the vessel with a dilation motion. The second robot gripper then proceeds to insert a shunt into the vessel phantom (a model of the blood vessel) with a chamfer tilt followed by a screw motion. Results suggest that AVSI achieves a high success rate even with tight tolerances and varying vessel orientations up to 30{\deg}. Supplementary material, dataset, videos, and visualizations can be found at https://sites.google.com/berkeley.edu/autolab-avsi.

==> figures/experimental_setup.tex <==
\begin{figure}[h]
\centering
\begin{tabular}{cc}
\frame{\includegraphics[width=.56\columnwidth]{images/Scene_fig.pdf}} &
\frame{\includegraphics[width=.375\columnwidth, trim= 0 80 0 0, clip]{images/vessels.png}}
\end{tabular}
\caption{\textbf{Experimental Setup.}   }
\label{fig:setup}
\end{figure}

==> tables/ablation.tex <==
\begin{table*}[!htbp]
\centering
% \vspace{-0.2cm}
\resizebox{\textwidth}{!}{
 \begin{tabular}{ c c c c c c c c }
\toprule
\textbf{Vessel orientation} & \textbf{Shunt outer diameter} & \textbf{Avg trial time} & \textbf{Successes} & \textbf{Attempts} & \textbf{Success Rate} & \multicolumn{2}{c}{\textbf{Failure Modes}} \\ 
\cmidrule{7-8}
\textit{(deg. from horizontal)} & \textit{(mm)} & \textit{(s)} & & & \textit{(\%)} & (D) & (S) \\
\midrule
\multirow{2}*{0} & 8 & 14.5 & 19 & 20 & 95 & 0 & 1 \\
& 14 & 14.4 & 16 & 20 & 80 & 0 & 4 \\
\hline
\multirow{2}*{15} & 8 & 15.0 & 18 & 20 & 90 & 1 & 1 \\
& 14 & 14.7 & 18 & 20 & 90 & 0 & 2 \\
\hline
\multirow{2}*{30} & 8 & 13.8 & 17 & 20 & 85 & 1 & 2 \\
& 14 & 14.8 & 10 & 20 & 50 & 0 & 10 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation Results:} Success rate and mean trial time for shunt insertion using our proposed method, with varying shunt and vessel configurations. We track two failure modes: (D) dilation failure and (S) shunt insertion failure.
}
\label{table:ablation_results}
% \vspace{-0.85cm}
\end{table*}

==> tables/non_baselines.tex <==
\begin{table*}[!htbp]
\centering
\resizebox{\textwidth}{!}{
 \begin{tabular}{c c c c c c c}
\toprule
\textbf{Shunt outer diameter} & \textbf{Avg trial time} & \textbf{Successes} & \textbf{Attempts} & \textbf{Success Rate} & \multicolumn{2}{c}{\textbf{Failure Modes}} \\ 
\cmidrule{6-7}
\textit{(mm)} & \textit{(s)} & & & \textit{(\%)} & (D) & (S) \\
\midrule
8 & 14.5 & 19 & 20 & 95 & 0 & 1 \\
14 & 14.4 & 16 & 20 & 80 & 0 & 4 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Results:} Success rate and mean trial time for shunt insertion using our proposed method. We track two failure modes: (D) dilation failure and (S) shunt insertion failure.
}
\label{table:non_baseline_results}
\end{table*}


==> tables/perception_ablation.tex <==
\begin{table*}[h]
\centering
% \vspace{-0.2cm}
\resizebox{\columnwidth}{!}{
 \begin{tabular}{ c c c c c c c c c }
\toprule
\textbf{Experiment} & \textbf{Vessel angle} & \textbf{Shunt outer diameter} & \textbf{Successes} & \textbf{Attempts} & \textbf{Success Rate} & \textbf{Avg trial time} & \multicolumn{2}{c}{\textbf{Failure Modes}} \\ 
\cmidrule{8-9}
& \textit{(deg)} & \textit{(mm)} & & & \textit{(\%)} & \textit{(s)} & (D) & (S) \\
\midrule
\multirow{2}*{No Dilation} & \multirow{2}*{0} & 8 & 20 & 20 & \textbf{100} & 9.0 & 0 & 0 \\
& & 14 & 0 & 20 & 0 & 10.1 & 0 & 20 \\
\midrule
Dilation Only & \multirow{2}*{0} & 8 & 19 & 20 & \textbf{95} & 13.7 & 1 & 0 \\
(No Screw Motion) & & 14 & 1 & 20 & 5 & 13.9 & 0 & 19 \\
\midrule
& \multirow{2}*{0} & 8 & 19 & 20 & \textbf{95} & 14.5 & 0 & 1 \\
& & 14 & 16 & 20 & \textbf{80} & 14.4 & 0 & 4 \\
\cmidrule{2-9}
Dilation + & \multirow{2}*{15} & 8 & 18 & 20 & \textbf{90} & 15.0 & 1 & 1 \\
Screw Motion & & 14 & 18 & 20 & \textbf{90} & 14.7 & 0 & 2 \\
\cmidrule{2-9}
& \multirow{2}*{30} & 8 & 17 & 20 & \textbf{85} & 13.8 & 1 & 2 \\
& & 14 & 10 & 20 & 50 & 14.8 & 0 & 10 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Experiment Results:} Success rate and mean trial time for shunt insertion with varying shunt with and without using dilation and screw motion, and including a vessel angle ablation. We track two failure modes: (D) dilation failure and (S) shunt insertion failure. 
}
\vspace{10pt}
\label{table:experiments}
% \vspace{-0.85cm}
\end{table*}
